Correcting the Contamination of Second-order Spectra: Improving H{\alpha} Measurements in Reverberation Mapping Campaigns

Long-term spectroscopic monitoring campaigns on active galactic nuclei (AGNs) provide a wealth of information about its interior structure and kinematics. However, a number of the observations suffer from the contamination of second-order spectra (SOS) which will introduce some undesirable uncertainties at the red side of the spectra. In this paper, we test the effect of SOS and propose a method to correct it in the time domain spectroscopic data using the simultaneously observed comparison stars. Based on the reverberation mapping (RM) data of NGC 5548 in 2019, one of the most intensively monitored AGNs by the Lijiang 2.4 m telescope, we find that the scientific object, comparison star, and spectrophotometric standard star can jointly introduce up to similar to 30% SOS for Grism 14. This irregular but smooth SOS significantly affects the flux density and profile of the emission line, while having little effect on the light curve. After applying our method to each spectrum, we find that the SOS can be corrected effectively. The deviation between corrected and intrinsic spectra is similar to 2%, and the impact of SOS on time lag is very minor. This method makes it possible to obtain the H alpha RM measurements from archival data provided that the spectral shape of the AGN under investigation does not have a large change.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

